High-Level Synthesis of Efficient Pipelines with Visibility Control

High-level synthesis (HLS) raises the abstraction of hardware design from concurrent register-transfer level (RTL). Among the forms of parallelism HLS exploits, pipelining demands fine-grained control over pipeline structure and hazard resolution to achieve competitive power, performance, and area (PPA). However, existing tools either lack such control or sacrifice sequential semantics to provide it. We present an HLS tool that embeds fine-grained pipeline control in a sequential programming model while generating synchronization logic only where needed to resolve the pipeline's potential hazards. The tool builds on visibility control, a novel programming abstraction that unifies hazard resolution techniques including stalling, bypassing, speculation, deferred commit, and register renaming. We evaluate on in-order RISC-V cores, histograms, and an AES accelerator. On RISC-V cores, we implement stall, bypass, speculation, and register renaming; on histograms, we implement scheduling strategies that previously required RTL or concurrent programming models. Compiled pipelines outperform HLS tools with sequential semantics and achieve PPA comparable to hand-written RTL.

==> setup.tex <==
\makeatletter%
\@ifundefined{basedir}{%
	\newcommand\basedir{}%
}{}%
\makeatother%

\makeatletter%



\usepackage{url}
\usepackage{datetime}
\usepackage{xspace}
\usepackage{wasysym}
\usepackage{mathpartir}
\usepackage{dashbox}
\usepackage[inline]{enumitem}
\setlist{leftmargin=5.5mm,topsep=2mm}
\setlist[enumerate]{label=\textbf{(\arabic*)}}
\usepackage{colortbl}
\usepackage{tikz}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{positioning}
\usepackage{tcolorbox}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{booktabs}%
\newlist{tabitemize}{itemize}{1}
\setlist[tabitemize]{leftmargin=2.5mm,label=\textbullet,nosep,after=\strut}
\usepackage{tabularx}
\usepackage[inkscapearea=page,inkscape=false]{svg}
\usepackage{minted}

\usepackage{wasysym}
\usepackage{fontawesome5}
\usepackage{marvosym}
\usepackage{diagbox}

\usepackage{algorithm}
\usepackage{./algpseudocodex} %

\usepackage{bytefield}

\usepackage{pifont}
\usepackage{adjustbox}        %
\usepackage{threeparttable}   %

\usepackage{upquote}
\usepackage{kotex}
\usepackage{multicol}

\usepackage{wrapfig}
\usepackage{esvect}
\MakeRobust{\vv}

\usepackage{changepage}
\usepackage{amsmath}

\usepackage{lipsum}

\usepackage{siunitx}
\sisetup{group-separator = {,}}


\usepackage{\basedir pftools}

\setlength{\textfloatsep}{11pt plus 2pt minus 4pt}
\setlength{\floatsep}{8pt plus 2pt minus 2pt}
\setlength{\intextsep}{8pt plus 2pt minus 2pt}
\captionsetup{skip=7pt}

\usepackage[nameinlink]{cleveref}

\definecolor{CodeBg}{gray}{0.98}
\newminted{rust}{bgcolor=CodeBg,fontsize=\footnotesize,linenos=true,breaklines,numbersep=4pt,xleftmargin=10pt}
\newmintinline{rust}{}

\newtheorem{reqthm}{Requirement}
\newtheorem{stthm}{Observation}
\newtheorem{case}{Case}

\definecolor{StringRed}{rgb}{.637,0.082,0.082}
\definecolor{CommentGreen}{rgb}{0.0,0.55,0.3}
\definecolor{KeywordBlue}{rgb}{0.0,0.3,0.55}
\definecolor{HighlightColor}{rgb}{0.0,0.0,0.0}


\definecolor{grey}{rgb}{0.5,0.5,0.5}
\definecolor{red}{rgb}{1,0,0}
\definecolor{darkgreen}{rgb}{0.0,0.7,0.0}

\definecolor{lightgreen2}{rgb}{0.71, 0.84, 0.65}

\crefdefaultlabelformat{\textcolor{ACMPurple}{#2#1}#3}

\crefname{section}{\textcolor{ACMPurple}{\S{}}}{\textcolor{ACMPurple}{\S{}}\!}
\crefformat{section}{\textcolor{ACMPurple}{#2\S{}#1#3}}
\Crefname{section}{Section}{Sections}
\Crefformat{section}{\textcolor{ACMPurple}{\S{}#2#1#3}}
\crefrangelabelformat{section}{\textcolor{ACMPurple}{#3#1#4}--\textcolor{ACMPurple}{#5#2#6}}

\Crefname{figure}{\textcolor{ACMPurple}{\text{Figure}}}{\textcolor{ACMPurple}{\text{Figures}}}
\crefname{figure}{\textcolor{ACMPurple}{\text{Fig.}}}{\textcolor{ACMPurple}{\text{Figs.}}}
\Crefname{table}{\textcolor{ACMPurple}{\text{Table}}}{\textcolor{ACMPurple}{\text{Tables}}}
\crefname{table}{\textcolor{ACMPurple}{\text{Table}}}{\textcolor{ACMPurple}{\text{Tables}}}

\crefname{algorithm}{\textcolor{ACMPurple}{\text{Algorithm} {}}}{\textcolor{ACMPurple}{\text{Algorithm} {}}\!}
\crefformat{algorithm}{\textcolor{ACMPurple}{#2\text{Algorithm} {}#1#3}}
\Crefname{algorithm}{\textcolor{ACMPurple}{\text{Algorithm}}}{\textcolor{ACMPurple}{\text{Algorithms}}}
\Crefformat{algorithm}{\textcolor{ACMPurple}{\text{Algorithm} {}#2#1#3}}
\crefrangelabelformat{algorithm}{\textcolor{ACMPurple}{#3#1#4--#5#2#6}}

\crefname{corollary}{\text{Corollary}}{\text{corollaries}}
\Crefname{corollary}{\text{Corollary}}{\text{Corollaries}}
\crefname{lemma}{\text{Lemma}}{\text{Lemmas}}
\Crefname{lemma}{\text{Lemma}}{\text{Lemmas}}
\crefname{theorem}{\text{Theorem}}{\text{Theorems}}
\Crefname{theorem}{\text{Theorem}}{\text{Theorems}}
\crefname{proposition}{\text{Prop.}}{\text{Propositions}}
\Crefname{proposition}{\text{Proposition}}{\text{Propositions}}
\crefname{definition}{\text{Def.}}{\text{Definitions}}
\Crefname{definition}{\text{Definition}}{\text{Definitions}}
\Crefname{reqthm}{\textcolor{ACMPurple}{\text{Requirement}}}{\textcolor{ACMPurple}{\text{Requirements}}}
\crefname{reqthm}{\textcolor{ACMPurple}{\text{Requirement}}}{\textcolor{ACMPurple}{\text{Requirements}}}
\Crefname{stthm}{\textcolor{ACMPurple}{\text{Observation}}}{\textcolor{ACMPurple}{\text{Observations}}}
\crefname{stthm}{\textcolor{ACMPurple}{\text{Observation}}}{\textcolor{ACMPurple}{\text{Observations}}}

\crefname{appendix}{\S{}}{\S{}\!}
\crefformat{appendix}{#2\S{}#1#3}
\Crefname{appendix}{Appendix}{Appendices}
\Crefformat{appendix}{\S{}#2#1#3}

\definecolor{amethyst}{rgb}{0.6, 0.4, 0.8}
\definecolor{blue-violet}{rgb}{0.54, 0.17, 0.89}
\definecolor{TokenLabelBg}{HTML}{D9D2E9}


\newcommand{\code}[1]{\texttt{#1}}
\DeclareRobustCommand{\api}[1]{\texttt{#1}}
\newcommand{\changed}[1]{\emph{\textcolor{KeywordBlue}{#1}}}
\newcommand{\eqdef}{\stackrel{\triangle}{=}}
\newcommand{\circled}[1]{{\footnotesize {\Circled{#1}}}}
\newcommand{\tokenlabel}[1]{%
	\tikz[baseline=(tok.base)]{%
		\node[
			draw=black,
			line width=0.7pt,
			rounded corners=2pt,
			fill=TokenLabelBg,
			inner xsep=2pt,
			inner ysep=0pt
		] (tok) {\strut \texttt{#1}};%
	}%
}

\newcommand{\parhead}[1]{\noindentparagraph{\textbf{#1}.}}

\newcommand{\dominates}{\ensuremath{\xrightarrow{dom}}}
\newcommand{\loopnest}{\ensuremath{\xrightarrow{nested}}}
\newcommand{\earlier}{\ensuremath{\prec}}
\newcommand{\earlierstatic}{\ensuremath{\prec_{\text{static}}}}
\newcommand{\leadstoforward}{\ensuremath{\leadsto_{E_f}}}

\newcommand{\aka}{a.k.a.\xspace}
\newcommand{\eg}{\emph{e.g.}\xspace}
\newcommand{\ie}{\emph{i.e.}\xspace}
\newcommand{\resp}{resp.\xspace}

\newcommand{\shakeflow}{\textsc{ShakeFlow}}
\newcommand{\bits}[1]{\ensuremath{\textsf{Bits}~{#1}}}
\newcommand{\unidir}{\ensuremath{\textsf{U}}}
\newcommand{\validready}{\ensuremath{\textsf{Vr}}}
\newcommand{\porttyp}[3]{\ensuremath{\textsf{PhT}_{{#1},{#2},{#3}}}}
\newcommand{\hazard}[3]{\ensuremath{\langle \mathsf{payload}: {#1}, \mathsf{bypass}: {#2}, \mathsf{ready}: {#3} \rangle}}
\newcommand{\hazardabbr}[3]{\ensuremath{\langle {#1}, {#2}, {#3} \rangle}}
\newcommand{\modt}[2]{\ensuremath{\langle \mathsf{i}: {#1}, \mathsf{e}: {#2} \rangle}}
\newcommand{\modtabbr}[2]{\ensuremath{\langle {#1}, {#2} \rangle}}
\newcommand{\port}[3]{\ensuremath{\textsf{Ch}_{#1}~{#2}~{#3}}}
\newcommand{\access}[2]{\ensuremath{\textsf{Acc}~{#1}~{#2}}}
\newcommand{\md}{\ensuremath{\textsf{Md}}}
\newcommand{\sm}[1]{\ensuremath{\textsf{Sm}_{#1}}}
\newcommand{\wire}[1]{\ensuremath{\textsf{Wr}~{#1}}}
\newcommand{\idx}[1]{\ensuremath{\textsf{Idx}~{#1}}}
\newcommand{\field}[1]{\ensuremath{\textsf{Fld}~{#1}}}
\newcommand{\x}[1]{\ensuremath{\textsf{X}_{#1}}}
\newcommand{\const}[2]{\ensuremath{\textsf{Const}_{#1}~{#2}}}
\newcommand{\var}[2]{\ensuremath{\textsf{Var}_{#1}~{#2}}}
\newcommand{\fsm}[4]{\ensuremath{\textsf{Fsm}_{{#1},{#2}}~{#3}~{#4}}}
\newcommand{\instm}[2]{\ensuremath{\textsf{DeclM}_{#1}~{#2}}}
\newcommand{\compm}[3]{\ensuremath{\langle \mathsf{t}: {#1}, \mathsf{e}: {#2}, \mathsf{comp}: {#3} \rangle}}
\newcommand{\compmabbr}[3]{\ensuremath{\langle {#1}, {#2}, {#3} \rangle}}
\newcommand{\monad}[1]{\ensuremath{\textsf{B}~{#1}}}
\newcommand{\tlist}[1]{\ensuremath{\textsf{list}~{#1}}}
\newcommand{\mret}[1]{\ensuremath{\textsf{return}~{#1}}}
\newcommand{\mbind}[2]{\ensuremath{\textsf{bind}~{#1}~{#2}}}
\newcommand{\mbuild}[1]{\ensuremath{\textsf{build}~{#1}}}
\newcommand{\mcomb}[2]{\ensuremath{\textsf{comb}~{#1}~{#2}}}
\newcommand{\app}{\ensuremath{\mathbin{+\!+}}}
\newcommand{\ready}{\ensuremath{\mathsf{ready}}}
\newcommand{\depto}{\ensuremath{\rightsquigarrow}}
\newcommand{\ndepto}{\ensuremath{\not\rightsquigarrow}}


\newcommand{\Stall}{\ensuremath{\boldsymbol{\times}}} %
\newcommand{\AddrStall}{\ensuremath{\boldsymbol{\triangle}}} %
\newcommand{\Bypass}{\ensuremath{\boldsymbol{\rightarrow}}} %
\newcommand{\MemAccess}{\ensuremath{\boldsymbol{\oplus}}} %


\newcommand{\sdecl}{\ensuremath{S_{\mathsf{decl}}}}
\newcommand{\sstore}{\ensuremath{S_{\mathsf{store}}}}
\newcommand{\sstorei}[1]{\ensuremath{S^{#1}_{\mathsf{store}}}}
\newcommand{\spub}{\ensuremath{S_{\mathsf{pub}}}}
\newcommand{\sbatch}{\ensuremath{S_{\mathsf{batch}}}}
\newcommand{\sload}{\ensuremath{S_{\mathsf{load}}}}
\newcommand{\sspec}{\ensuremath{S_{\mathsf{spec}}}}


\newcommand{\maydeclare}{\ensuremath{\mathsf{MayDeclare}}}
\newcommand{\nodeclare}{\ensuremath{\mathsf{NoDeclare}}}
\newcommand{\mayload}{\ensuremath{\mathsf{MayLoad}}}
\newcommand{\noload}{\ensuremath{\mathsf{NoLoad}}}
\newcommand{\declared}{\ensuremath{\mathsf{Declared}}}
\newcommand{\tentative}{\ensuremath{\mathsf{Tentative}}}
\newcommand{\sealed}{\ensuremath{\mathsf{Sealed}}}
\newcommand{\idle}{\ensuremath{\mathsf{Idle}}} %
\newcommand{\speculative}{\ensuremath{\mathsf{Speculative}}}
\newcommand{\determined}{\ensuremath{\mathsf{Determined}}}

\newcommand{\SPS}{\ensuremath{\mathsf{SPS}}}
\newcommand{\LoopIndex}{\ensuremath{\mathsf{LoopIndex}}}
\newcommand{\LocalMemory}{\ensuremath{\mathsf{LocalMemory}}}
\newcommand{\PublishedView}{\ensuremath{\mathsf{PublishedView}}}
\newcommand{\TokenValue}{\ensuremath{\mathsf{TokenValue}}}
\newcommand{\pirctx}{\ensuremath{K}}
\newcommand{\pirsegrel}[1]{\ensuremath{[\![ #1 ]\!]_{\pirctx}}}
\newcommand{\pircomp}{\ensuremath{\mathbin{;}}}
\newcommand{\pirlive}[2]{\ensuremath{\mathsf{live}_{#1}(#2)}}
\newcommand{\combrel}[1]{\ensuremath{[\![ #1 ]\!]_{\mathsf{Comb}}}}
\newcommand{\rustrel}[1]{\ensuremath{[\![ #1 ]\!]_{\mathsf{Rust}}}}
\newcommand{\piperel}[1]{\ensuremath{[\![ #1 ]\!]_{\mathsf{Pipe}}}}
\newcommand{\lpo}{\ensuremath{\prec_P}}


\algrenewcommand\algorithmicindent{1.0em}
\newcommand*{\Continue}{\textbf{continue}}
\newcommand*{\Break}{\textbf{break}}

\newcommand{\automation}{{\tiny\faCog}}
\newcommand{\manual}{\ding{45}}
\newcommand{\cmark}{{\color{CommentGreen}\ding{51}}} %
\newcommand{\xmark}{{\color{StringRed}\ding{55}}} %
\newcommand{\pmark}{{\(\LEFTcircle\)}} %

\makeatletter
\newcounter{algorithmicH}%
\let\oldalgorithmic\algorithmic
\renewcommand{\algorithmic}{%
	\stepcounter{algorithmicH}%
	\oldalgorithmic}%
\renewcommand{\theHALG@line}{ALG@line.\thealgorithmicH.\arabic{ALG@line}}
\makeatother


\newcommand*{\todotmpl}[3]{\textcolor{#2}{[{#1}: {#3}]}}
\newcommand*{\todo}[1]{\todotmpl{todo}{blue}{#1}}
\newcommand*{\jeehoon}[1]{\todotmpl{jeehoon}{purple}{#1}}
\newcommand*{\minseong}[1]{\todotmpl{minseong}{cyan}{#1}}
\newcommand*{\jungin}[1]{\todotmpl{jungin}{darkgreen}{#1}}
\newcommand*{\claude}[1]{\todotmpl{claude}{purple}{#1}}
\newcommand*{\claudetodo}[1]{\todotmpl{claudetodo}{teal}{#1}}
\newcommand*{\woojin}[1]{\todotmpl{woojin}{violet}{#1}}
\newcommand*{\zhao}[1]{\todotmpl{zhao}{violet}{#1}}
\newcommand*{\jaewoo}[1]{\todotmpl{jaewoo}{teal}{#1}}
\newcommand*{\janggun}[1]{\todotmpl{janggun}{violet}{#1}}
\newcommand*{\seungmin}[1]{\todotmpl{seungmin}{brown}{#1}}
\newcommand*{\grammarly}[1]{\todotmpl{Grammarly}{red}{#1}}
\newcommand*{\review}[1]{\todotmpl{Review}{violet}{#1}}

\newcommand*{\revision}{\jeehoon{REVISED SO FAR}}

\newcommand*{\reviewuntil}{\jungin{PLEASE REVIEW UNTIL THIS POINT}}


\newcommand\closure[1]{\ensuremath{\overline{#1}}}
\newcommand{\mcomp}[3]{\ensuremath{{#2} \bowtie_{#1} {#3}}}
\newcommand{\pto}{\ensuremath{\rightharpoonup}}
\newcommand{\hzflow}{\textsc{HazardFlow}\xspace}

\newcommand{\relstep}[3]{\ensuremath{#1 ~\vdash~ \big\langle #2 \big\rangle \rightarrow_{\mathsf{step}} \big\langle #3 \big\rangle}}

\newcommand{\relstepsimple}[8]{\relstep{#1}{#2,\; #3,\; #4,\; #5}{#6,\; #7,\; #8}}

\newcommand{\reltoksimple}[4]{\ensuremath{#1 ~\vdash~ \big\langle #2 \big\rangle
		\rightarrow_{\mathsf{tok}} \big\langle #3,\; #4 \big\rangle}}

\newcommand{\reltokfull}[7]{\ensuremath{#1 ~\vdash~ \big\langle #2,\; #3,\; #4 \big\rangle
		\rightarrow_{\mathsf{tok}} \big\langle #5,\; #6,\; #7 \big\rangle}}

\newcommand{\nreltokfull}[7]{\ensuremath{#1 ~\vdash~ \big\langle #2,\; #3,\; #4 \big\rangle
		\nrightarrow_{\mathsf{tok}} \big\langle #5,\; #6,\; #7 \big\rangle}}



